Merging Cluster Collaboration: A Panchromatic Atlas of Radio Relic Mergers

Golovich et al. 2017b presents an optical imaging and spectroscopic survey of 29 radio relic merging galaxy clusters. In this paper, we study this survey to identify substructure and quantify the dynamics of the mergers. Using a combined photometric and spectroscopic approach, we identify the minimum number of substructures in each system to describe the galaxy populations and estimate the line of sight velocity difference between likely merging subclusters. We find that the line-of-sight velocity components of the mergers are typically small compared with the maximum three dimensional relative velocity (usually $<1000$ km s$^{-1}$ and often consistent with zero). This suggests that the merger axes of these systems are generally in or near the plane of the sky matching findings in magneto-hydrodynamical simulations. In 28 of the 29 systems we identify substructures in the galaxy population aligned with the radio relic(s) and presumed associated merger induced shock. From this ensemble, we identify eight systems to include in a `gold' sample that is prime for further observation, modeling, and simulation study. Additional papers will present weak lensing mass maps and dynamical modeling for each merging system, ultimately leading to new insight into a wide range of astrophysical phenomena at some of the largest scales in the universe.

==> table2.tex <==
\begin{tabular}{lllll}
Cluster 					&	Filter		&	Date					&	Seeing (arcsec)		&	Exposure (s)\\
\hline
1RXS J060313.4+421231		&	g		&	2014 February 25		&	0.57				&	720	\\
1RXS J060313.4+421231		&	r		&	2014 February 25		&	0.57				&	2880\\
1RXS J060313.4+421231		&	i		&	2014 February 25		&	0.50				&	720	\\
Abell 523					&	g		&	2014 February 26		&	1.00				&	720	\\
Abell 523					&	r		&	2014 February 26		&	0.78				&	2880\\
Abell 746					&	g		&	2014 February 26		&	0.88				&	720	\\
Abell 746					&	r		&	2014 February 26		&	1.01				&	2880\\
Abell 1240				&	g		&	2014 February 25		&	0.67				&	720	\\
Abell 1240				&	r		&	2014 February 25		&	0.58				&	2880\\
Abell 1300				&	g		&	2014 February 26		&	0.89				&	720	\\
Abell 1300				&	r		&	2014 February 26		&	0.88				&	2160	\\
Abell 2061				&	g		&	2013 July 13			&	0.68				&	720\\
Abell 2061				&	r		&	2013 July 13			&	0.67				&	2520	\\
Abell 2061				&	i		&	2013 July 13			&	0.60				&	2676	\\
Abell 2061				&	i		&	2014 February 26		&	0.65				&	720  \\
Abell 3365				&	g		&	2014 February 25		&	0.97				&	720 \\
Abell 3365				&	r		&	2014 February 25		&	0.71				&	2880	\\
Abell 3365				&	i		&	2014 February 25		&	0.62				&	720 \\
Abell 3411					&	g		&	2014 February 25		&	0.80				&	720	\\
Abell 3411					&	r		&	2014 February 25		&	0.82				&	2880\\
Abell 3411					&	i		&	2014 February 25		&	0.77				&	720	\\
CIZA J2242.8+5301			&	g		&	2013 July 13			&	0.63				&	720	\\
CIZA J2242.8+5301			&	i		&	2013 July 13			&	0.55				&	3400	\\
MACS J175201.5+444046	&	g		&	2013 July 13			&	0.62				&	720	\\
MACS J175201.5+444046	&	r		&	2013 July 13			&	0.64				&	1440\\
MACS J175201.5+444046	&	i		&	2013 July 13			&	0.63				&	2520	\\
MACS J175201.5+444046	&	i		&	2014 February 26		&	0.73				&	1260	\\
PLCKESZ G287.0+32.9		&	g		&	2014 February 26		&	0.81				&	720	\\
PLCKESZ G287.0+32.9		&	r		&	2014 February 26		&	0.97				&	2880\\
PSZ1 G108.18-11.53		&	g		&	2015 September 12		&	0.65				&	1440 \\
PSZ1 G108.18-11.53		&	r		&	2015 September 12		&	0.55				&	2520\\
RXC J1053.7+5452			&	g		&	2014 February 26		&	0.83				&	720	\\
RXC J1053.7+5452			&	r		&	2014 February 26		&	0.92				&	720	\\
RXC J1314.4-2515			&	g		&	2014 February 25		&	0.86				&	720\\
RXC J1314.4-2515			&	r		&	2014 February 25		&	0.71				&	2880	\\
RXC J1314.4-2515			&	NB814	&	2014 February 25		&	0.77				&	1000	\\
ZwCl 0008.8+5215			&	g		&	2013 July 13			&	0.52				&	720\\
ZwCl 0008.8+5215			&	r		&	2013 July 13			&	0.57				&	2880	\\
ZwCl 1447+2619			&	g		&	2014 February 26		&	0.91				&	720	\\
ZwCl 1447+2619			&	r		&	2014 February 26		&	0.76				&	2880\\
ZwCl 1447+2619			&	i		&	2014 February 26		&	0.55				&	720	\\
ZwCl 1856+6616			&	g		&	2015 September 12		&	0.70				&	720 \\
ZwCl 1856+6616			&	r		&	2015 September 12		&	0.65				&	2520\\
ZwCl 2341+0000			&	g		&	2013 July 13			&	0.49				&	720	\\
ZwCl 2341+0000			&	r		&	2013 July 13			&	0.50				&	2880\\
\end{tabular}

==> table3.tex <==
\begin{tabular}{lllll}
Cluster 					&	Filter		&	Date									&	Exposure (s)\\
\hline
Abell 115					&	V		&	2003 September 25, 2005 October 03		&	1530	\\
Abell 115					&	i		&	2005 October 03						&	2100\\
Abell 521					&	V		&	2001 October 14						&	1800\\
Abell 521					&	R		&	2001 October 15						&	1620\\
Abell 781					&	V		&	2010 March 14, 15						&	3360\\
Abell 781					&	i		&	2010 March 15							&	2160\\
Abell 2034				&	g		&	2005 April 11							&	720\\
Abell 2034				&	R		&	2005 April 11, 2007 June 19				&	12880\\
Abell 2163				&	V		&	2009 April 30							&	2100\\
Abell 2163				&	R		&	2008 April 07							&	4500\\
Abell 2255				&	B		&	2007 August 14							&	1260\\
Abell 2255				&	R		&	2007 August 14							&	2520\\
Abell 2345				&	V		&	2010 June 10, 2010 November 10			&	3600\\
Abell 2345				&	i		&	2005 October 03						&	2100\\
Abell 2744				&	B		&	2013 July 16							&	2100\\
Abell 2744				&	R		&	2013 July 15							&	3120\\
MACS J1149				&	V		&	2003 April 05							&	2520\\
MACS J1149				&	R		&	2003 April 05, 2005 March 05, 2010 March 18	&	5490\\
\end{tabular}

==> table4.tex <==
\begin{tabular}{llllll}
Slitmask 		&	Date				&	Target Imaging	&	Exposure (s)	&	Wavelength (\AA)&	Slits\\
\hline
1RXSJ0603-1	&	2013 January 16	&	WFC		&	3000		&	6200		&	105\\
1RXSJ0603-2	&	2013 January 16	&	WFC		&	3000		&	6200		&	100\\
1RXSJ0603-3	&	2013 September 5	&	WFC		&	3600		&	7000		&	98\\
1RXSJ0603-4	&	2013 September 5	&	WFC		&	3600		&	7000		&	87\\
A115-1		&	2014 June 22		&	SDSS	&	2500		&	6900		&	176\\
A115-2		&	2014 June 23		&	SDSS	&	2400		&	6900		&	142\\
A523-1		&	2013 January 16	&	WFC		&	3000		&	6200		&	99\\
A523-2		&	2013 December 4	&	WFC		&	2700		&	6200		&	94\\
A523-3		&	2015 February 16	&	WFC		&	2700		&	6300		&	111\\
A746-1		&	2013 January 16	&	SDSS	&	3600		&	6200		&	110\\
A1240-1		&	2013 December 3	&	SDSS	&	2700		&	6850		&	120\\
A1240-2		&	2015 February 16	&	SDSS	&	2700		&	6820		&	164\\
A1612-1		&	2015 February 16	&	SDSS	&	1200		&	6750		&	140\\
A2034-1		&	2013 July 14		&	SDSS	&	2700		&	6700		&	158\\
A2443-1		&	2014 June 22		&	SDSS	&	2400		&	6400		&	153\\
A2443-2		&	2014 June 23		&	SDSS	&	2400		&	6400		&	163\\
A3365-1		&	2013 January 16	&	WFC		&	2700		&	6200		&	68\\
A3365-2		&	2013 January 16	&	WFC		&	2400		&	6200		&	66\\
A3365-3		&	2013 December 3	&	WFC		&	2700		&	6300		&	63\\
A3365-4		&	2013 December 4	&	WFC		&	2700		&	6300		&	66\\
A3365-5		&	2015 February 16	&	SC		&	2700		&	6200		&	160\\
A3411-1		&	2013 December 3	&	WFC		&	2700		&	6650		&	132\\
A3411-2		&	2013 December 3	&	WFC		&	2700		&	6650		&	127\\
A3411-3		&	2013 December 4	&	WFC		&	2700		&	6650		&	128\\
A3411-4		&	2013 December 4	&	WFC		&	2700		&	6650		&	131\\
A3411-5		&	2015 December 13	&	SC		&	3600		&	6650		&	142\\
CIZAJ2242-1	&	2013 July 14		&	WFC		&	2700		&	6700		&	148\\
CIZAJ2242-2	&	2013 July 14		&	WFC		&	2700		&	6700		&	126\\
CIZAJ2242-3	&	2013 September 5	&	SC		&	2700		&	7000		&	90\\
CIZAJ2242-4	&	2013 September 5	&	SC		&	2700		&	7000		&	106\\
MACSJ1752-1	&	2013 July 14		&	SDSS	&	2700		&	6700		&	155\\
MACSJ1752-2	&	2013 July 14		&	SDSS	&	2700		&	6700		&	119\\
MACSJ1752-3	&	2013 September 5	&	SDSS	&	3600		&	7000		&	114\\
MACSJ1752-4	&	2013 September 5	&	SDSS	&	2700		&	7000		&	118\\
PLCKG287-1	&	2015 February 16	&	SC		&	3900		&	7950		&	207\\
PLCKG287-2	&	2015 February 16	&	SC		&	2700		&	7950		&	185\\
PLCKG287-3	&	2015 February 16	&	SC		&	2700		&	7950		&	193\\
PSZ1G108-1	&	2014 June 22		& 	DSS		&	1800		&	7400		&	198\\
PSZ1G108-2	&	2014 June 23		& 	DSS		&	1800		&	7650		&	168\\
RXCJ1053-1	&	2013 January 16	&	SDSS	&	2803		&	6200		&	113\\
RXCJ1053-2	&	2013 December 3	&	SDSS	&	2700		&	6200		&	84\\
RXCJ1053-3	&	2013 December 4	&	SDSS	&	2430		&	6200		&	98\\
RXCJ1053-4	&	2015 February 16	&	SC		&	2700		&	6200		&	141\\
RXCJ1314-1	&	2015 February 16	&	SC		&	2520		&	7120		&	196\\
RXCJ1314-2	&	2015 February 16	&	SC		&	2520		&	7120		&	207\\
ZwCl0008-1	&	2013 January 16	&	WFC		&	2063		&	6200		&	81\\
ZwCl0008-2	&	2013 July 14		&	WFC		&	2700		&	6700		&	81\\
ZwCl0008-3	&	2013 September 5	&	WFC		&	2700		&	7000		&	75\\
ZwCl0008-4	&	2013 September 5	&	WFC		&	3600		&	7000		&	73\\
ZwCl1447-1	&	2014 June 22		&	SDSS	&	1520		&	7850		&	149\\
ZwCl1447-2	&	2014 June 23		&	SDSS	&	1053		&	7850		&	138\\
ZwCl1856-1	&	2014 June 22		& 	DSS		&	1800		&	7400		&	150\\
ZwCl1856-2	&	2014 June 23		& 	DSS		&	1800		&	7400		&	101\\
ZwCl2341-1	&	2013 July 14		&	SDSS	&	2700		&	6700		&	130\\
ZwCl2341-2	&	2013 July 14		&	SDSS	&	2700		&	6700		&	131\\
ZwCl2341-3	&	2013 September 5	&	SDSS	&	2700		&	7000		&	148\\
\end{tabular}

==> table6.tex <==
\clearpage
\LongTables
\begin{deluxetable*}{lllll}
\tablecaption{Priors for potential subclusters as deemed such by the routine discussed in \S \ref{subsec:gmm} for 29 merging galaxy clusters.} 
\tablehead{
\colhead{Cluster} & 
\colhead{Halo} & 
\colhead{X Position (Mpc)}&
\colhead{Y Position (Mpc)} &
\colhead{LOS Velocity (1000 km s$^{-1}$)}}
\startdata
1RXS J0603 	& a  	& [$-0.58$,$-0.36$] 	& [$+0.32$,$+0.57$]	& [$-2.5$,$-0.50$]\\
		     	& b	& [$-0.24$,$-0.02$] 	& [$+0.10$,$+0.37$]	& [$-0.50$,$+0.50$]\\
			& c	& [$-0.67$,$-0.33$] 	& [$-0.78$,$-€0.14$]	& [$+0.75$,$+2.5$]\\
			& d	& [$+0.11$,$+0.33$] & [$-1.1$,$-0.75$]	& [$-2.0$,$-1.0$]\\
\hline
A115			& a	& [$-0.45$,$-0.23$] 	& [$+0.06$,$+0.38$]	& [$+0.05$,$+1.3$]\\
			& b	& [$-0.10$,$+0.13$] 	& [$-0.69$,$-€0.42$]	& [$-0.90$,$+0.30$]\\
\hline
A521	 		& a	& [$-0.76$,$-0.51$]	& [$+0.26$,$+0.45$]	& [$-1.4$,$-0.20$]\\
			& b	& [$-0.20$,$+0.04$]	& [$+0.08$,$+0.29$]	& [$+0.05$,$+0.55$]\\
			& c	& [$-0.07$,$+0.18$]	& [$-0.12$,$+0.04$]	& [$+0.20$,$+0.90$]\\
			& d	& [$+0.19$,$+0.42$]	& [$-0.51$,$-0.26$]	& [$-1.4$,$+0.50$]\\	
\hline
A523			& a	& [$+0.04$,$+0.16$] 	& [$+0.38$,$+0.51$]	& [$-0.42$,$+0.10$]\\
			& b	& [$-0.18$,$-0.05$] 	& [$-0.27$,$-€0.08$]	& [$-0.15$,$+0.65$]\\
\hline
A781	 		& a  	& [$-0.35$,$-0.08$] 	& [$+0.61$,$+0.94$]	& [$+0.80$,$+2.0$]\\
		     	& b	& [$-1.19$,$-0.92$] 	& [$+0.14$,$+0.43$]	& [$+0.60$,$+1.8$]\\
			& c	& [$-0.22$,$-0.05$] 	& [$-0.05$,$-€0.27$]	& [$-0.20$,$+1.0$]\\
			& d	& [$+1.2$,$+1.4$] 	& [$-0.41$,$-0.11$]	& [$-1.9$,$-0.7$]\\
\hline
A1240		& a	& [$-0.22$,$0$] 	& [$+0.27$,$+0.54$]	& [$-0.65$,$+0.60$]\\
			& b	& [$-0.14$,$+0.08$] 	& [$-0.74$,$-0.45$]	& [$-1.0$,$0$]\\
\hline
A1300 		& a  	& [$-0.35$,$-0.07$] 	& [$+0.10$,$+0.31$]	& [$+0.10$,$+1.0$]\\
		     	& b	& [$-0.04$,$+0.24$] 	& [$-0.19$,$0$]		& [$-1.3$,$-0.50$]\\
			& c	& [$-0.39$,$-0.03$] 	& [$-0.43$,$-€0.31$]	& [$+0.20$,$+0.80$]\\
\hline
A1612		& a	& [$-0.67$,$-0.47$] 	& [$+0.01$,$+0.25$]	& [$-0.45$,$+0.55$]\\
			& b	& [$+0.16$,$+0.38$] 	& [$-0.42$,$-€0.08$]	& [$-0.55$,$+0.45$]\\
\hline
A2034 		& a  	& [$-0.04$,$0.09$] 	& [$+0.47$,$+0.62$]	& [$-0.20$,$+0.85$]\\
		     	& b	& [$0$,$+0.13$] 	& [$-0.14$,$+0.01$]	& [$-1.1$,$-0.05$]\\
			& c	& [$-0.38$,$-0.25$] 	& [$-0.39$,$-€0.23$]	& [$+0.60$,$+1.7$]\\
\hline
A2061		& a	& [$-0.21$,$+0.05$] 	& [$-0.05$,$+0.40$]	& [$-0.30$,$+0.85$]\\
			& b	& [$-0.38$,$-0.22$] 	& [$-0.48$,$-0.22$]	& [$-0.70$,$+0.45$]\\
\hline
A2163 		& a  	& [$+0.04$,$+0.27$] 	& [$+0.95$,$+1.2$]	& [$-0.90$,$+0.35$]\\
		     	& b	& [$+0.06$,$+0.26$] & [$-0.25$,$-0.06$]	& [$-0.35$,$+0.40$]\\
			& c	& [$-0.73$,$-0.53$] 	& [$-0.38$,$-€0.13$]	& [$-0.60$,$+0.20$]\\
			& d	& [$-0.26$,$-0.05$] 	& [$-0.51$,$-0.33$]	& [$-.20$,$+0.95$]\\
\hline
A2255 		& a  	& [$-0.33$,$-0.21$] 	& [$+0.01$,$+0.15$]	& [$+0.25$,$+1.35$]\\
		     	& b	& [$-0.40$,$-0.29$] 	& [$-0.06$,$+0.07$]	& [$-2.4$,$-1.3$]\\
			& c	& [$+0.09$,$+0.22$] 	& [$-0.13$,$+0.11$]	& [$-1.7$,$-0.3$]\\
\hline
A2345 		& a  	& [$-1.4$,$-1.1$] 	& [$-0.07$,$+0.46$]	& [$-0.65$,$+0.40$]\\
		     	& b	& [$+0.21$,$+0.40$] 	& [$-0.18$,$+0.08$]	& [$-0.10$,$+0.95$]\\
			& c	& [$-0.54$,$-0.29$] 	& [$-0.75$,$-0.35$]	& [$-1.1$,$0$]\\
\hline
A2443		& a	& [$-0.24$,$-0.10$] 	& [$-0.07$,$+0.10$]	& [$-0.75$,$+0.60$]\\
			& b	& [$-0.02$,$+0.15$] 	& [$-0.30$,$-0.14$]	& [$-0.75$,$+0.75$]\\
\hline
A2744 		& a	& [$+0.01$,$+0.28$]	& [$+0.38$,$+0.65$]	& [$-1.4$,$-0.95$]\\
			& b	& [$-0.43$,$-0.16$]	& [$+0.15$,$+0.38$]	& [$-1.5$,$-0.90$]\\
			& c	& [$+0.18$,$+0.46$]	& [$-0.19$,$-0.01$]	& [$-2.0$,$-1.2$]\\
			& d	& [$+0.27$,$+0.58$]	& [$-0.32$,$-0.19$]	& [$+2.5$,$+3.1$]\\	
			& e	& [$-0.55$,$-0.10$]	& [$-0.31$,$-0.21$]	& [$-1.2$,$-0.65$]\\
\hline
A3365 		& a  	& [$+0.39$,$+0.63$] 	& [$-0.02$,$+0.38$]	& [$-1.0$,$+0.25$]\\
		     	& b	& [$-1.0$,$-0.83$] 	& [$-0.21$,$+0.18$]	& [$+1.0$,$+3.0$]\\
			& c	& [$-0.58$,$-0.34$] 	& [$-0.34$,$+0.03$]	& [$-1.0$,$+0.25$]\\	
\hline
A3411 		& a  	& [$-0.26$,$-0.10$] 	& [$+1.3$,$+1.5$]	& [$-0.60$,$+0.60$]\\
		     	& b	& [$-0.39$,$-0.21$] 	& [$+0.34$,$+0.67$]	& [$-0.25$,$+1.0$]\\
			& c	& [$+0.16$,$+0.35$] 	& [$-0.83$,$-0.50$]	& [$-1.0$,$+0.25$]\\	
\hline
CIZAJ2242	& a	& [$-0.13$,$+0.14$] 	& [$+0.50$,$+1.1$]	& [$-1.0$,$+1.0$]\\
			& b	& [$-0.48$,$-0.24$] 	& [$-0.73$,$-0.37$]	& [$-1.0$,$+1.0$]\\
\hline
MACSJ1149	& a  	& [$-0.46$,$-0.03$] 	& [$+0.38$,$+0.95$]	& [$+2.2$,$+3.5$]\\
		     	& b	& [$-0.38$,$+0.01$] 	& [$-0.16$,$+0.39$]	& [$-1.3$,$+0.50$]\\
			& c	& [$+0.26$,$+0.65$] 	& [$-0.92$,$-0.48$]	& [$-1.5$,$0$]\\	
\hline
MACSJ1752	& a	& [$+0.13$,$+0.48$] 	& [$-0.05$,$+0.33$]	& [$-0.40$,$+0.40$]\\
			& b	& [$-0.75$,$-0.38$] 	& [$-0.64$,$-0.11$]	& [$+0.05$,$+0.95$]\\
\hline
PLCKG287	& a	& [$-0.44$,$-0.12$] 	& [$+0.12$,$+0.44$]	& [$-1.0$,$+1.0$]\\
			& b	& [$+0.53$,$+0.90$] 	& [$-2.5$,$-2.0$]	& [$-1.9$,$-1.1$]\\
\hline
RXCJ1053	& a  	& [$-0.53$,$-0.42$] 	& [$0$,$+0.18$]	& [$-0.60$,$+0.25$]\\
		     	& b	& [$-0.11$,$0$] 	& [$-0.17$,$-0.02$]	& [$-0.15$,$+0.85$]\\
			& c	& [$+0.68$,$+0.78$] 	& [$-0.48$,$-0.32$]	& [$-1.0$,$+0.10$]\\	
\hline
RXCJ1314	& a	& [$-0.10$,$+0.13$] 	& [$+0.05$,$+0.30$]	& [$-0.90$,$-0.40$]\\
			& b	& [$-0.67$,$-0.44$] 	& [$-0.06$,$+0.20$]	& [$+0.10$,$+0.80$]\\
\hline
ZwCl0008		& a	& [$+0.43$,$+0.56$] 	& [$+0.10$,$+0.26$]	& [$+0.10$,$+0.90$]\\
			& b	& [$-0.57$,$-0.44$] 	& [$-0.20$,$-0.02$]	& [$-0.40$,$+0.60$]\\
\hline
ZwCl1447		& a	& [$+0.08$,$+0.39$] 	& [$+0.31$,$+0.59$]	& [$-0.40$,$+1.0$]\\
			& b	& [$-0.30$,$+0.06$] 	& [$-0.54$,$-0.24$]	& [$-1.0$,$+0.40$]\\
\hline
A2744 		& a	& [$-0.28$,$-0.02$]	& [$+0.59$,$+0.85$]	& [$0$,$+1.5$]\\
			& b	& [$-0.58$,$-0.33$]	& [$+0.40$,$+0.71$]	& [$-0.60$,$+0.30$]\\
			& c	& [$-0.21$,$+0.05$]	& [$+0.04$,$+0.25$]	& [$-0.20$,$+1.2$]\\
			& d	& [$+0.11$,$+0.37$]	& [$-0.75$,$-0.37$]	& [$-0.70$,$+0.10$]\\	


==> table7.tex <==

1RXSJ0603		&	1	& -		& 18		& 0.160 	& 147\\
			&	2	& ab		& 38 		& 0.093 	&178\\
			&	3	& ac		& 66		& 0.078 	& 250\\
			&	4	& ad		& 87		& 0.121 	& 165\\
			&	5	& bc		& 28		& 0.086 	& 199\\
			&	6	& bd 		& 0		& 0.105 	& 8.73\\
			&	7	& cd		& 75		& 0.070 	& 219\\
			&	8	& abc	& 0 		& 0.072 	& 242\\
			&	9	& abd	& 0		& 0.084 	& 4.36\\
			&	10	& acd	& 8		& 0.083 	& 62.7\\
			&	11	& bcd	& 1		& 0.052	& 444\\
			&	12	& abcd	&14		& 0.074	& 0\\
\hline
A115			&	1	& - 	 	&  0		& 0.170	& 33.3  \\
			&	2	& ab		& 26		& 0.093	& 0 \\ 
\hline
A521			&	1	& -		& 0		& 0.161 	& 15.4 \\
			&	2	& ab		& 10		& 0.092 	& 16.9\\
			&	3	& ac		& 9		& 0.098 	& 30.1\\
			&	4	& ad		& 0		& 0.109 	& 28.2\\
			&	5	& bc		& 5		& 0.067 	& 24.0\\
			&	6	& bd 		& 16		& 0.102 	& 0\\
			&	7	& cd		&  0		& 0.100 	& 21.7\\
			&	8	& abc	& 11		& 0.051 	& 46.7\\
			&	9	& abd	& 9 		& 0.073 	& 21.9\\
			&	10	& acd	& 0		& 0.092 	& 20.0\\
			&	11	& bcd	& 7		& 0.072 	& 21.7\\
			&	12	& abcd	& 0		& 0.055 	& 45.3\\
\hline
A523			&	1	& -		& 10		& 0.126 	& 2.55  \\
			&	2	& ab		& 15		& 0.108 	& 0	\\
\hline
A746			&	1	& -		& 1		& 0.088 	& - \\
\hline
A781			&	1	& -		& 300	& 0.187 	& 64.9\\
			&	2	& ab		& 322	& 0.161 	& 185\\
			&	3	& ac		& 288	& 0.166 	& 196\\
			&	4	& ad		& 203	& 0.188 	& 19.4\\
			&	5	& bc		& 281	& 0.162 	& 181\\
			&	6	& bd		& 192	& 0.182 	& 18.4\\
			&	7	& cd		& 152	& 0.189 	& 10.4\\
			&	8	& abc	& 285	& 0.114 	& 194\\
			&	9	& abd	& 159	& 0.122 	& 18.6\\
			&	10	& acd	& 165	& 0.139 	& 3.92\\
			&	11	& bcd	& 116	& 0.136 	& 8.14\\
			&	12	& abcd	& 128	& 0.100 	& 0\\
\hline
A1240		&	1	& -		& 8		& 0.161 	& 22.1\\
			&	2	& ab		& 8		& 0.112 	& 0\\
\hline
A1300		&	1	& -		& 23		&  0.131 	& 16.4 \\
			&	2	& ab		& 9		&  0.104 	& 75.3\\
			&	3	& ac		& 10	 	&  0.077 	& 62.9\\
			&	4	& bc		& 0		&  0.085 	& 5.10\\
			&	5	& abc	& 0		&  0.071 	& 0 \\
\hline
A1612		&	1	& -		& 0		&  0.161	& 29.5\\
			&	2	& ab	 	& 17		&  0.119	&0 \\
\hline
A2034		&	1	& -		& 27		&  0.117 	& 38.3 \\
			&	2	& ab		& 0		&  0.066	& 14.2\\
			&	3	& ac		& 27	 	&  0.073	& 59.8\\
			&	4	& bc		& 0		&  0.068 	& 33.6\\
			&	5	& abc	& 0		&  0.058 	& 0\\			
\hline
A2061		&	1	& -		& 20 		& 0.119	& 10.5 \\
			&	2	& ab		& 6		& 0.077	& 0 \\
\hline
A2163		&	1	& -		&  224	& 0.228 	& 0 \\
			&	2	& ab		& 184	& 0.126	& 9.51\\
			&	3	& ac		& 230	& 0.124 	& 25.1\\
			&	4	& ad		& 230	& 0.118	& 33.8\\
			&	5	& bc		& 225	& 0.111	& 37.0\\
			&	6	& bd		& 234	& 0.095	& 31.4\\
			&	7	& cd		& 250	& 0.087 	& 35.6\\
			&	8	& abc	& 182	& 0.081 	& 4.62\\
			&	9	& abd	& 55		& 0.051 	& 13.6\\
			&	10	& acd	& 258	& 0.081 	& 44.9 \\
			&	11	& bcd	& 107	& 0.061	& 94.1\\
			&	12	& abcd	& 36		& 0.045	& 145\\
\hline
A2255		&	1	& -		& 0		& 0.195 	& 0 \\
			&	2	& ab		& 33		& 0.113	& 64.2\\
			&	3	& ac		& 0	 	& 0.099	& 55.8\\
			&	4	& bc		& 37		& 0.084	& 110\\
			&	5	& abc	& 0		& 0.077	& 79.9\\	
\hline
A2345		&	1	& -		& 0		& 0.221 	& 0  \\
			&	2	& ab		& 0 		& 0.153	& 12.5\\
			&	3	& ac		& 0	 	& 0.169	& 157\\
			&	4	& bc		& 0		& 0.094	& 39.4\\
			&	5	& abc	& 0		& 0.088	& 41.2\\
\hline
A2443		&	1	& -		& 0		& 0.222	& 4.61\\
			&	2	& ab		& 0		& 0.145	& 0	\\
\hline
A2744		&	1	& -		& 225	& 0.188	& 19.1	\\
			&	2	& ab		& 225	& 0.157	& 42.4	\\
			&	3	& ac		& 199	& 0.158	& 22.1	\\
			&	4	& ad		& 198	& 0.165	& 16.7	\\
			&	5	& ae		& 218	& 0.166	& 38.1	\\
			&	6	& bc		& 192	& 0.160	& 19.0	\\
			&	7	& bd		& 197	& 0.149	& 11.9	\\
			&	8	& be		& 227	& 0.145	& 12.2	\\
			&	9	& cd		& 206	& 0.158	& 26.6	\\
			&	10	& ce		& 203	& 0.159	& 24.0	\\
			&	11	& de		& 191	& 0.078	& 23.8	\\
			&	12	& abc	& 72		& 0.073	& 93.2	\\
			&	13	& abd	& 59		& 0.081	& 101	\\
			&	14	& abe	& 70		& 0.107	& 125	\\
			&	15	& acd	& 88  	& 0.080	& 92.1	\\
			&	16	& ace	& 179	& 0.082	& 12.5	\\
			&	17	& ade	& 74		& 0.084	& 9.33	\\
			&	18	& bcd	& 57		& 0.073	& 17.9	\\
			&	19	& bce	& 72		& 0.061	& 4.55	\\
			&	20	& bde	& 58		& 0.067	& 5.53	\\
			&	21	& cde	& 89		& 0.074	& 84.1	\\
			&	22	& abcd	& 18		& 0.067	& 129	\\
			&	23	& abce	&59		& 0.076	& 66.1	\\
			&	24	& abde	& 68		& 0.078	& 108	\\
			&	25	& acde	& 44		& 0.070	& 0	\\
			&	26	& bcde	& 55		& 0.065	& 4.31	\\
			&	27	& abcde	& 32		& 0.057	& 83.8	\\
\hline
A3365		&	1	& -		& 3		& 0.188 	& 55.5  \\
			&	2	& ab		& 1 		& 0.151	& 43.4\\
			&	3	& ac		& 0	 	& 0.144	& 25.8\\
			&	4	& bc		& 0		& 0.172	& 103\\
			&	5	& abc	& 0		& 0.099	& 0\\
\hline
A3411		&	1	& -		& 0		& 0.201 	& 140  \\
			&	2	& ab		& 0 		& 0.147	& 290\\
			&	3	& ac		& 0	 	& 0.134	& 172\\
			&	4	& bc		& 0		& 0.159	& 0\\
			&	5	& abc	& 0		& 0.101	& 27.7\\
\hline
CIZAJ2242	&	1	& -		& 0		& 0.201	& 25.7\\
			&	2	& ab		& 0		& 0.177	& 0	\\			
\hline
MACSJ1149	&	1	& -		& 25		& 0.157 	& 55.5  \\
			&	2	& ab		& 32 		& 0.104	& 43.4\\
			&	3	& ac		& 69	 	& 0.093	& 25.8\\
			&	4	& bc		& 40		& 0.107	& 103\\
			&	5	& abc	& 20		& 0.083	& 0\\		
\hline
MACSJ1752	&	1	& -		& 44		& 0.091	& 4.41\\
			&	2	& ab		& 14		& 0.071	& 0	\\
\hline
PLCKG287	&	1	& -		& 162	& 0.273	& 1.72\\
			&	2	& ab		& 190	& 0.140	& 0	\\
\hline
PSZ1G108	&	1	& -		& 0		& 0.105	& - \\
\hline
RXCJ1053	&	1	& -		& 12		& 0.188 	& 12.9  \\
			&	2	& ab		& 10		& 0.089	& 0 \\
			&	3	& ac		& 9 		& 0.106	& 55.8\\
			&	4	& bc		& 16		& 0.092	& 13.8\\
			&	5	& abc	& 3		& 0.065	& 33.3\\	
\hline
RXCJ1314	&	1	& -		& 0		& 0.156	& 4.44\\
			&	2	& ab		& 0		& 0.093	& 0	\\
\hline
ZwCl0008		&	1	& -		& 7		& 0.104	& 3.71\\
			&	2	& ab		& 5		& 0.097	& 0 \\
\hline	
ZwCl1447		&	1	& -		& 26		& 0.091	& 0 \\
			&	2	& ab		& 6		& 0.070	& 8.01\\
\hline
ZwCl1856		&	1	& -		& 5		& 0.168	& 1.21\\
			&	2	& ab		& 3		& 0.098	& 0 \\
\hline	
ZwCl2341		&	1	& -		&  12		& 0.173 	& 82.1 \\
			&	2	& ab		&  44		& 0.082	& 249\\
			&	3	& ac		&  0		& 0.104 	& 118\\
			&	4	& ad		&  0 		& 0.129	& 4.80\\
			&	5	& bc		&  14		& 0.087	& 150\\
			&	6	& bd		&  0		& 0.114	& 10.9\\
			&	7	& cd		& 18		& 0.121 	& 30.7\\
			&	8	& abc	&  23		& 0.067 	& 137\\
			&	9	& abd	&  21		& 0.095 	& 0\\
			&	10	& acd	&  8		& 0.042 	& 55.2 \\
			&	11	& bcd	&  0		& 0.078	& 23.3\\
			&	12	& abcd	&  0 		& 0.071	& 32.1\\
